PIR: Photometric Inverse Rendering with Shading Cues Modeling and Surface Reflectance Regularization

This paper addresses the problem of inverse rendering from photometric images. Existing approaches for this problem suffer from the effects of self-shadows, inter-reflections, and lack of constraints on the surface reflectance, leading to inaccurate decomposition of reflectance and illumination due to the ill-posed nature of inverse rendering. In this work, we propose a new method for neural inverse rendering. Our method jointly optimizes the light source position to account for the self-shadows in images, and computes indirect illumination using a differentiable rendering layer and an importance sampling strategy. To enhance surface reflectance decomposition, we introduce a new regularization by distilling DINO features to foster accurate and consistent material decomposition. Extensive experiments on synthetic and real datasets demonstrate that our method outperforms the state-of-the-art methods in reflectance decomposition.

==> tables/equations.tex <==
\newcommand{\normal}{\boldsymbol{n}}
\newcommand{\point}{\boldsymbol{x}}

%\resizebox{0.48\textwidth}{!}{
    %\large
\renewcommand{\arraystretch}{1.3}
    \begin{tabular}{llll}
        \toprule
        Notation & Example\\
        \midrule
         Fraction &  $\frac{1}{a}$ \\
         Max & $\max (a, 0 )$ \\
         Dimension & $\boldsymbol{x} \in \mathbb{R}^3$ \\
         Argmax  & $\mathop{\arg\max}_{a} f(ax)$ \\
         cos & $\cos(x)$ \\
         Hat/tilde & $\hat{\boldsymbol{x}}, \tilde{\boldsymbol{x}}$ \\
         Tensor operation & $\otimes$, \quad $\circ$, \quad $\odot$ \\ 
         Sum & $\sum_{i=1}^{N} x_i$ \\
         Approximation & $f(x) \approx g(x)$ \\
         Around & $\sim$100 \\
         Product & $\prod_{i=1}^{N} x_i$ \\
         Integral & $\int_{-\infty}^{+\infty} x_i$ \\
         Gradient & $\boldsymbol{n}(n) = \nabla o(\boldsymbol{x})/\|\nabla o(\boldsymbol{x})\|_2$ \\
         Parallel & $\mathcal{L} = \sum \| x_i - \hat{x}_i \|^2_2$ \\
         Set & $\{I_i | i=1,\dots, N \}$ \\
        \bottomrule
    \end{tabular}
%    }



==> tables/greek_letters.tex <==
    \resizebox{0.48\textwidth}{!}{
    \large
    \begin{tabular}{clclclclc}
        \toprule
        Symbol & \LaTeX  & Symbol & \LaTeX & Symbol & \LaTeX\\
        \midrule
$\alpha  $ & \textbackslash alpha   & $\kappa $ & \textbackslash kappa  & $\psi    $  & \textbackslash psi    \\
$\beta   $ & \textbackslash beta    & $\lambda$ & \textbackslash lambda & $\rho    $  & \textbackslash rho    \\
$\chi    $ & \textbackslash chi     & $\mu    $ & \textbackslash mu     & $\sigma  $  & \textbackslash sigma  \\
$\delta  $ & \textbackslash delta   & $\nu    $ & \textbackslash nu     & $\tau    $  & \textbackslash tau    \\
$\epsilon$ & \textbackslash epsilon & $ o     $ & \textbackslash o      & $\theta  $  & \textbackslash theta  \\
$\eta    $ & \textbackslash eta     & $\omega $ & \textbackslash omega  & $\upsilon$  & \textbackslash upsilon\\
$\gamma  $ & \textbackslash gamma   & $\phi   $ & \textbackslash phi    & $\xi     $  & \textbackslash xi     \\
$\iota   $ & \textbackslash iota    & $\pi    $ & \textbackslash pi     & $\zeta   $  & \textbackslash zeta   \\
\midrule
$ \digamma   $ & \textbackslash digamma    & $ \Delta $ & \textbackslash digamma    & $ \Theta   $  & \textbackslash Theta  \\
$ \varepsilon$ & \textbackslash varepsilon & $ \Gamma $ & \textbackslash varepsilon & $ \Upsilon $  & \textbackslash Upsilon\\
$ \varkappa  $ & \textbackslash varkappa   & $ \Lambda$ & \textbackslash varkappa   & $ \Xi      $  & \textbackslash Xi     \\
$ \varphi    $ & \textbackslash varphi     & $ \Omega $ & \textbackslash varphi     &               &         \\
$ \varpi     $ & \textbackslash varpi      & $ \Phi   $ & \textbackslash varpi      & $ \aleph   $  & \textbackslash aleph  \\
$ \varrho    $ & \textbackslash varrho     & $ \Pi    $ & \textbackslash varrho     & $ \beth    $  & \textbackslash beth   \\
$ \varsigma  $ & \textbackslash varsigma   & $ \Psi   $ & \textbackslash varsigma   & $ \daleth  $  & \textbackslash daleth \\
$ \vartheta  $ & \textbackslash vartheta   & $ \Sigma $ & \textbackslash vartheta   & $ \gimel   $  & \textbackslash gimel  \\
        \bottomrule
    \end{tabular}
    }



==> tables/res_cd.tex <==
% \resizebox{0.48\textwidth}{!}{
%     %\Large
% \begin{tabular}{l||*{1}{c}|*{3}{c}|*{3}{c}|*{3}{c}}
%     \toprule
%     % & \multicolumn{1}{c|}{Distance}
%     & \multicolumn{1}{c|}{Roughness}
%     & \multicolumn{3}{c|}{Diffuse Albedo}
%     & \multicolumn{3}{c|}{Specular Albedo}
%     & \multicolumn{3}{c}{View Synthesis RGB}\\
%     Method & MSE $\times 10^{-3}$ & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS \\
%     \midrule
%     % NeuS \cite{luan2021unified} & 23.7630 \\
%     WildLight \cite{cheng2023wildlight} & 106.32
%     & 25.631 & 0.9189 & 0.1186
%     & 17.357 & 0.8353 & 0.2016
%     & 29.167 & 0.9300 & 0.0929 \\
%     IRON \cite{iron-2022} & 1.8402
%     & 33.175 & 0.9730 & 0.0432
%     & 25.809 & 0.8496 & 0.1645
%     & 29.053 & 0.9604 & 0.0558
%     \\
%     Ours & \textbf{0.8808}
%     & \textbf{35.777} & \textbf{0.9805} & \textbf{0.0331}
%     & \textbf{29.716} & \textbf{0.9136} & \textbf{0.1065}
%     & \textbf{31.891} & \textbf{0.9700} & \textbf{0.0488} \\
%     \bottomrule
% \end{tabular}
% }

\resizebox{0.48\textwidth}{!}{
\large
\begin{tabular}{*{4}{c}}
    \toprule
    Method & Average CD ($\times 10^{-3}$) \\
    \midrule
    NeuS & 3.325 \\
    IRON & 3.106 \\
    Ours & \textbf{2.784} \\
    \bottomrule
\end{tabular}
}
\captionof{table}{Average chamfer distance on synthetic data.}
\label{tab:geo}







==> tables/res_collocated_synthetic.tex <==
\resizebox{\textwidth}{!}{
    %\Large
\begin{tabular}{l||*{3}{c}|*{3}{c}|*{3}{c}|*{3}{c}|*{3}{c}}
    \toprule
    & \multicolumn{3}{c|}{\emph{Duck}} 
    & \multicolumn{3}{c|}{\emph{Maneki}}
    & \multicolumn{3}{c|}{\emph{Horse}}
    & \multicolumn{3}{c|}{\emph{Marble Bowl}}
    & \multicolumn{3}{c}{\emph{Dragon}} \\
    Method & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS \\
    \midrule
    % PS-NeRF \cite{yang2022psnerf} \\
    % TensoIR \cite{jin2023tensoir} \\
    % NeILF++ \cite{zhang2023neilf++} \\
    % WildLight \cite{cheng2023wildlight} \\		
    IRON \cite{iron-2022} & 39.868 & 0.9957 & 0.0251 & 33.999 & 0.9764 & 0.0300 & 36.165 & 0.9863 & 0.0262 & & & & 28.822 & 0.9460 & 0.0679 \\
    
    Ours w/o $\boldsymbol{f}_{\text{dino}}$ & 40.000 & 0.9952 & 0.0238 & \textbf{34.838} & \textbf{0.9787} & 0.0285 & 37.062 & 0.9894 & 0.0253 & & & & \textbf{29.286} & 0.9460 & 0.0685 \\
    
    Ours & \textbf{41.686} & \textbf{0.9962} & \textbf{0.0230} & 34.777 & 0.9785 & \textbf{0.0282} & \textbf{37.530} & \textbf{0.9910} & \textbf{0.0249} & & & & 29.169 & \textbf{0.9471} & \textbf{0.0684} \\
    \bottomrule
\end{tabular}
}


==> tables/res_inter_reflection.tex <==
\resizebox{0.48\textwidth}{!}{
    %\Large
\begin{tabular}{*{3}{c}||*{3}{c}}
    \toprule
    Inter-refl. & VQ Reg. & Sparisty Reg. & PSNR & SSIM & LPIPS \\
    \midrule
    & & & 29.2520 & 0.9749 & 0.0424 \\
    \checkmark & & & 30.0787 & 0.9765 & 0.0397 \\
    \checkmark & \checkmark & & \textbf{30.2812} & \textbf{0.9780} & \textbf{0.0386} \\
    \checkmark & & \checkmark & 29.7268 & 0.9752 & 0.0418 \\
    \bottomrule
\end{tabular}
}



==> tables/res_real.tex <==
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{3}{c}|*{3}{c}|*{3}{c}|*{3}{c}}
    \toprule
    & \multicolumn{3}{c|}{\emph{dragon} (DRV)}
    & \multicolumn{3}{c|}{\emph{girl}}
    & \multicolumn{3}{c|}{\emph{pony}}
    & \multicolumn{3}{c}{Average} \\
    Method & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS \\
    \midrule
    % NeuS & \\
    WildLight \cite{cheng2023wildlight}
    & xxx & xxx & xxx
    & xxx & xxx & xxx \\
    TensoIR \cite{jin2023tensoir}
    & xxx & xxx & xxx
    & xxx & xxx & xxx \\
    IRON \cite{iron-2022}
    & 30.920 & 0.9030 & 0.1384 
    & 24.339 & 0.8729 & 0.1356 
    & 29.269 & 0.9150 & 0.1095
    & 28.177 & 0.8970 & 0.1278 \\
    Ours
    & \textbf{00.000} & \textbf{0.0000}& \textbf{xxx} 
    & \textbf{xxx} & \textbf{xxx}& \textbf{xxx} \\
    \bottomrule
\end{tabular}
}



==> tables/two_subtables.tex <==
\newcommand{\PSNRT}{PSNR\xspace}
\newcommand{\VQM}{HDR-VQM\xspace}
\newcommand{\VDP}{HDR-VDP2\xspace}
\newcommand{\LowExposure}{Low-Exposure\xspace}
\newcommand{\MiddleExposure}{Middle-Exposure\xspace}
\newcommand{\HighExposure}{High-Exposure\xspace}
\newcommand{\AllExposure}{All-Exposure\xspace}

\makebox[\textwidth]{\small (a) Results on dataset A.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & \Scnd{40.00} & 73.70 & \Scnd{40.04} & \Scnd{70.08} & \Scnd{40.02} & 71.89 & \Scnd{76.22} 
                  & \Scnd{39.61} & 73.24 & \Frst{39.67} & \Frst{73.24} & \Frst{40.01} & 67.90 & \Frst{39.77} & 70.37 & 79.55 \\
    Method B      & 34.54 & 80.22 & 39.25 & 65.96 & 36.90 & 73.09 & 65.33 
                  & 36.51 & 77.78 & 37.45 & 69.79 & 39.02 & 64.57 & 37.66 & 70.71 & 70.13 \\
    Method C  & 39.79 & \Scnd{81.02} & 39.96 & 67.25 & 39.88 & \Scnd{74.13} & 73.84 
                  & 39.48 & \Scnd{78.13} & 38.43 & 70.08 & 39.60 & \Scnd{67.94} & 39.17 & \Scnd{72.05} & \Scnd{80.70} \\
    Ours          & \Frst{41.95} & \Frst{81.03} & \Frst{40.41} & \Frst{71.27} & \Frst{41.18} & \Frst{76.15} & \Frst{78.84}
                  & \Frst{40.00} & \Frst{78.66} & \Scnd{39.27} & \Scnd{73.10} & \Scnd{39.99} & \Frst{69.99} & \Scnd{39.75} & \Frst{73.92} & \Frst{82.87} \\
    \bottomrule
\end{tabular}
}

\vspace{0.5em}
\makebox[\textwidth]{\small (b) Results on dataset B.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & 37.73 & 74.05 & 45.71 & 66.67 & 41.72 & 70.36 & 85.33 
                  & 37.53 & 72.03 & 36.38 & 65.37 & 34.73 & 62.24 & 36.21 & 66.55 & 84.43 \\
    Method B      & 36.41 & 85.68 & \Scnd{49.89} & \Scnd{69.90} & 43.15 & 77.79 & 78.92 
                  & 36.43 & 77.74 & 39.80 & \Scnd{67.88} & \Scnd{43.03} & \Scnd{64.74} & 39.75 & \Scnd{70.12} & 87.93 \\
    Method C  & \Scnd{39.94} & \Scnd{86.77} & 49.49 & 69.04 & \Scnd{44.72} & \Scnd{77.91} & \Scnd{87.16} 
                  & \Scnd{38.34} & \Scnd{78.04} & \Scnd{41.21} & 66.07 & 42.66 & 64.01 & \Scnd{40.74} & 69.37 & \Scnd{89.36}\\
    Ours          & \Frst{40.83} & \Frst{86.84} & \Frst{50.10} & \Frst{71.33} & \Frst{45.46} & \Frst{79.09} & \Frst{87.40} 
                  & \Frst{38.77} & \Frst{78.11} & \Frst{41.47} & \Frst{68.49} & \Frst{43.24} & \Frst{65.08} & \Frst{41.16} & \Frst{70.56} & \Frst{89.56}\\
    \bottomrule
\end{tabular}
}

